Learning Multi-level Weight-centric Features for Few-shot Learning

Few-shot learning is currently enjoying a considerable resurgence of interest, aided by the recent advance of deep learning. Contemporary approaches based on weight-generation scheme delivers a straightforward and flexible solution to the problem. However, they did not fully consider both the representation power for unseen categories and weight generation capacity in feature learning, making it a significant performance bottleneck. This paper proposes a multi-level weight-centric feature learning to give full play to feature extractor's dual roles in few-shot learning. Our proposed method consists of two essential techniques: a weight-centric training strategy to improve the features' prototype-ability and a multi-level feature incorporating a mid- and relation-level information. The former increases the feasibility of constructing a discriminative decision boundary based on a few samples. Simultaneously, the latter helps improve the transferability for characterizing novel classes and preserve classification capability for base classes. We extensively evaluate our approach to low-shot classification benchmarks. Experiments demonstrate our proposed method significantly outperforms its counterparts in both standard and generalized settings and using different network backbones.

==> author_bios.tex <==
\newpage
\noindent
\textbf{Author Biography}
\\
\textbf{Mingjiang Liang}
is currently pursuing a PhD from the University of Technology Sydney. She received her master degree from the Northwestern Polytechnical University. Her current research interest mainly focus on few-shot learning.
\\
\noindent
\textbf{Shaoli Huang}
received his Ph.D. degree under the supervision of Prof. Dacheng Tao from the University of Technology Sydney in 2017. He is a research fellow in UBTECH Sydney AI Centre at The University of Sydney. His research interests include deep learning, pose estimation, object detection, and fine-grained object recognition.
\\
\textbf{Shirui Pan} is a Senior Lecturer with the Department of Data Science & AI, Faculty of Information Technology, Monash University. Prior to this, he was a Lecturer with the Centre for Artificial Intelligence (CAI), School of Software, Faculty of Engineering and Information Technology, University of Technology Sydney(UTS). Shirui received his Ph.D degree in computer science from UTS, Australia. His research interests include data mining and machine learning, specialized in graph mining and network analysis.
\\
\textbf{Mingming Gong} a lecturer in Data Science at the School of Mathematics and Statistics, University of Melbourne (UoM). He is part of the Melbourne Deep Learning Group. His research interests lie in machine learning, artificial intelligence, and data science, especially in causal reasoning, transfer learning, and deep learning. He develop computational methods for causal reasoning from observational data and exploit causal knowledge to build more intelligent machine learning algorithms.

\\
\textbf{Wei Liu}
 an Associate Professor in Machine Learning, and the Director of Future Intelligence Research Lab, in the School of Computer Science, the University of Technology Sydney (UTS). He obtained his PhD degree in Machine Learning research at the University of Sydney (USyd). His current research focuses are adversarial machine learning, cybersecurity, game theory, multimodal machine learning, natural language processing, and intrusion detection. 
